Sources of Irreproducibility in Machine Learning: A Review

Background: Many published machine learning studies are irreproducible. Issues with methodology and not properly accounting for variation introduced by the algorithm themselves or their implementations are attributed as the main contributors to the irreproducibility.Problem: There exist no theoretical framework that relates experiment design choices to potential effects on the conclusions. Without such a framework, it is much harder for practitioners and researchers to evaluate experiment results and describe the limitations of experiments. The lack of such a framework also makes it harder for independent researchers to systematically attribute the causes of failed reproducibility experiments. Objective: The objective of this paper is to develop a framework that enable applied data science practitioners and researchers to understand which experiment design choices can lead to false findings and how and by this help in analyzing the conclusions of reproducibility experiments. Method: We have compiled an extensive list of factors reported in the literature that can lead to machine learning studies being irreproducible. These factors are organized and categorized in a reproducibility framework motivated by the stages of the scientific method. The factors are analyzed for how they can affect the conclusions drawn from experiments. A model comparison study is used as an example. Conclusion: We provide a framework that describes machine learning methodology from experimental design decisions to the conclusions inferred from them.

==> Sources of irreproducibility/parts_removed.tex <==
\section{Machine Learning Methodology}
\label{sec:machine_learning_methodology}
\citet{mitchell_1997} defines \emph{machine learning} as follows: a computer program is said to learn from experience \textit{E} with respect to some class of tasks \textit{T} and performance measure \textit{P}, if its performance at tasks in \textit{T} as measured by \textit{P} improves with experience \textit{E}.
Computer programs that learn are often called machine learning models or models for short. 


Progress in machine learning is to a large degree driven by empirical evidence, and \emph{model comparison} is the standard method to identify the best performing machine learning model for a given task \cite{melis_2017,sculley_2018,bouthillier_2019,dacrema_2021}.
A \emph{model comparison study} is an experiment of which the objective is to decide which of a set of models has better performance.
Hence, a model comparison identifies the subset \textit{S} of a given set of computer programs \textit{C} that performs task \textit{T} better according to measure \textit{P} after learning from the same experience \textit{E}.
For a computer program, or model, to be considered a clear winner of a model comparison, it should be significantly better than the model that was previously considered state-of-the-art for the given task \cite{sculley_2018}. 
The hypothesis that a model is significantly better than the other models in the comparison should be tested statistically \cite{cohen_1995}. 
Empirical evidence is given by conducting experiments where the competing models learn from the same experiences under the same conditions. 

Machine learning is typically described by three different paradigms: supervised learning, unsupervised learning and reinforcement learning \cite{mitchell_1997,russel_norvig_2020}. 
We will use supervised learning for our examples.% as it is the most common form of machine learning.

\emph{Supervised learning} is defined by \citet{russel_norvig_2020} in the following way:
experience is a given \emph{training set} (experience $E$) of $N$ example input-output pairs: $(x_1,y_1),(x_2,y_2),...(x_N,y_N)$ where each pair is generated by an unknown function $y=f(x)$. 
Machine learning is to discover a function $h$ that approximates the function $f$.
The function $h$ is a model drawn from a model class $H$. 
As we cannot expect $h(x_i)=y_i$ for each $x_i$, we search for a \emph{best-fit} model $h$ that minimizes the error rate, which is the proportion of times that $h(x) \neq y$ for an example $(x,y)$. 
To avoid cheating, the model should not have seen the test as part of the training, and therefore test data should be different from training data. 
This division between training and test data is the main principle of machine learning methodology.
A dataset is divided into three parts to find the best-fit model.
The training set is used to find candidate models while a \emph{validation set} used identify the best candidate models, and finally the \emph{test set} is used to do a final unbiased evaluation of the best model. 
Hyperparameters are parameters of the model class $H$, such as the order of a polynomial or the number of hidden layers in a deep neural network.
%Model comparison studies aim at identifying the best model class for a given task, and are typically done when introducing new model classes, which could include new deep learning architectures or modules. %Reference here?

\textbf{Example:} We now present an example from a classic model comparison study conducted by \citet{lecun_1998} that illustrates how the scientific method, see figure \ref{fig:scientific_method}, applies to machine learning. 
The example is simplified to only comprise parts of the study.
The goal of the study is to find out whether dense neural networks (DNN) or convolutional neural networks (CNN) are better at performing the task of assigning the numbers 0-9 to images of handwritten digits. 
The \emph{null hypothesis} is that CNNs do not perform better than DNNs and the \emph{alternative hypothesis} is that CNNs perform better at the classification task. 
The \emph{prediction} is that CNNs will perform better because of the convolutional layer that is specifically designed to deal with the variability of two dimensional shapes. 

The experiment is designed, which results in a study plan and an analysis plan. 
The \emph{study plan} specifies which data to use, such as combining two different datasets into the Modified NIST set, and specifies how to divide the data into training, validation and test sets. 
In the classic model study, no validation set was used as different hyperparameters are tested explicitly -- without a hyperparameter search. 
The training set contains 60 000 images while the test set contains 10 000 images.
The \emph{analysis plan} details how to evaluate the results by using error rate on the test set to declare the winner.

% Bør det hete ML models i fig 1?
%Ikke forklare overordnet, men konkret
The implementation of the experiment contains all the steps before executing the experiment on the test set so that the outcome can be analyzed. 
This includes collecting and \emph{pre-processing data}, which is to combine the two NIST datasets into one. 
The training dataset was pre-processed (augmented) by adding images that were distorted in different ways.
The MNIST dataset was famously published, but the augmented dataset was not. 
The DNN and CNN algorithms were implemented without relying on an open source library while \emph{initialization} of the experiment included the initialization of neural network weights was done  manually by hand as well more systematically for different parts. 
It is not clear whether the complete \emph{workflow} was automated or parts of it were done manually, as code is not shared.  
\emph{Ancillary software}, such as operating system, was not specified, but the \emph{hardware} was, as the experiment was executed on a Silicon Graphics Origin server with a 200 MHz F10000 processor.
Executing the training of the algorithms on the training data resulted in the two models $m_{DNN}$ $m_{CNN}$.

The \emph{outcome} is the classes [0-9] given to each image in the test set. 
It is not shared, but the \emph{analysis} is, which is the metric error rate (in \%) on the test set reported in a bar graph. 
The best DNN has an error rate of 2.95\% without training on distorted images and an error rate of 2.45\% when the distorted images are used while the best CNN (LeNet-5) has an error rate of 0.95\% that is reduced to 0.8\% when adding distortion. 
Non-neural network baselines were also reported, which includes SVM's among several others. 
The best baseline reported a result of 0.8\%.
The uncertainty is reported to be 0.1\% for all the error rates. 
However, it is not clear how the uncertainty is computed.
The alternative hypothesis is supported as the CNN is better than DNN taking the uncertainty into account.
However, the experiment cannot conclude what the state of the art is performance-wise, as the experiment has no clear winner given how close the error rate of the SVM and CNN are. 
Still, additional experiments show that the CNN runs faster and requires less memory, which are important properties when choosing algorithms. 
%\oeg{Should I integrate the six factors more explicitly in this example: Study design, algorithmic, implementation, observation, evaluation, documentation into this example.}




%A model comparison study is conducted where two machine learning models, $m_a$ and $m_b$, compete to identify which of them are better at performing a classification task. %$m_{DNN}$ $m_{CNN}$
%The hypothesis is that $m_a$ performs better than $m_b$ on the test dataset after being trained on the training dataset.
%10-fold cross validation is done to identify the best set of hyperparameters for each model.
%After identifying the best hyperparameters each of the models classify each image in the test set.
%Performance is measured using classification error.
%The experiment is run five times and the mean error and variance are reported.
%The strength of the evidence is measured through statistical hypothesis testing.
%The final results support the hypothesis in that $m_a$ performs significantly better than $m_b$.
%The conclusion from the original study was that it supports the hypothesis. 




%Things to discuss:
%- The task of the model comparison experiment => define properly in related to the definition
%- Data
%- ML methodology
% Engineering


% Stuff commented out: Draft ideas
%Machine learning methodology is developed around the notion that "an agent learns if it improves its performance after making observations about the world" \cite{russel_norvig_2020}. 
%In supervised learning, which is the most common form of machine learning algorithms, agents learn from input-output pairs and have to learn to map input to output, and its performance is measured using a performance metric such as error rate, that is the proportion of times where the agent fails to map the input to the output.



%artificial Intelligence, and machine learning by extension, is not only about studying the behavior of intelligent systems, but also to build them \cite{russel_norvig_2020}.


%While the performance of some systems are evaluated on their performance on real-world tasks, such as AlphaGo and Watson
%While some ML systems are built and evaluated 




==> parts_removed.tex <==
\section{Machine Learning Methodology}
\label{sec:machine_learning_methodology}
\citet{mitchell_1997} defines \emph{machine learning} as follows: a computer program is said to learn from experience \textit{E} with respect to some class of tasks \textit{T} and performance measure \textit{P}, if its performance at tasks in \textit{T} as measured by \textit{P} improves with experience \textit{E}.
Computer programs that learn are often called machine learning models or models for short. 


Progress in machine learning is to a large degree driven by empirical evidence, and \emph{model comparison} is the standard method to identify the best performing machine learning model for a given task \cite{melis_2017,sculley_2018,bouthillier_2019,dacrema_2021}.
A \emph{model comparison study} is an experiment of which the objective is to decide which of a set of models has better performance.
Hence, a model comparison identifies the subset \textit{S} of a given set of computer programs \textit{C} that performs task \textit{T} better according to measure \textit{P} after learning from the same experience \textit{E}.
For a computer program, or model, to be considered a clear winner of a model comparison, it should be significantly better than the model that was previously considered state-of-the-art for the given task \cite{sculley_2018}. 
The hypothesis that a model is significantly better than the other models in the comparison should be tested statistically \cite{cohen_1995}. 
Empirical evidence is given by conducting experiments where the competing models learn from the same experiences under the same conditions. 

Machine learning is typically described by three different paradigms: supervised learning, unsupervised learning and reinforcement learning \cite{mitchell_1997,russel_norvig_2020}. 
We will use supervised learning for our examples.% as it is the most common form of machine learning.

\emph{Supervised learning} is defined by \citet{russel_norvig_2020} in the following way:
experience is a given \emph{training set} (experience $E$) of $N$ example input-output pairs: $(x_1,y_1),(x_2,y_2),...(x_N,y_N)$ where each pair is generated by an unknown function $y=f(x)$. 
Machine learning is to discover a function $h$ that approximates the function $f$.
The function $h$ is a model drawn from a model class $H$. 
As we cannot expect $h(x_i)=y_i$ for each $x_i$, we search for a \emph{best-fit} model $h$ that minimizes the error rate, which is the proportion of times that $h(x) \neq y$ for an example $(x,y)$. 
To avoid cheating, the model should not have seen the test as part of the training, and therefore test data should be different from training data. 
This division between training and test data is the main principle of machine learning methodology.
A dataset is divided into three parts to find the best-fit model.
The training set is used to find candidate models while a \emph{validation set} used identify the best candidate models, and finally the \emph{test set} is used to do a final unbiased evaluation of the best model. 
Hyperparameters are parameters of the model class $H$, such as the order of a polynomial or the number of hidden layers in a deep neural network.
%Model comparison studies aim at identifying the best model class for a given task, and are typically done when introducing new model classes, which could include new deep learning architectures or modules. %Reference here?

\textbf{Example:} We now present an example from a classic model comparison study conducted by \citet{lecun_1998} that illustrates how the scientific method, see figure \ref{fig:scientific_method}, applies to machine learning. 
The example is simplified to only comprise parts of the study.
The goal of the study is to find out whether dense neural networks (DNN) or convolutional neural networks (CNN) are better at performing the task of assigning the numbers 0-9 to images of handwritten digits. 
The \emph{null hypothesis} is that CNNs do not perform better than DNNs and the \emph{alternative hypothesis} is that CNNs perform better at the classification task. 
The \emph{prediction} is that CNNs will perform better because of the convolutional layer that is specifically designed to deal with the variability of two dimensional shapes. 

The experiment is designed, which results in a study plan and an analysis plan. 
The \emph{study plan} specifies which data to use, such as combining two different datasets into the Modified NIST set, and specifies how to divide the data into training, validation and test sets. 
In the classic model study, no validation set was used as different hyperparameters are tested explicitly -- without a hyperparameter search. 
The training set contains 60 000 images while the test set contains 10 000 images.
The \emph{analysis plan} details how to evaluate the results by using error rate on the test set to declare the winner.

% Bør det hete ML models i fig 1?
%Ikke forklare overordnet, men konkret
The implementation of the experiment contains all the steps before executing the experiment on the test set so that the outcome can be analyzed. 
This includes collecting and \emph{pre-processing data}, which is to combine the two NIST datasets into one. 
The training dataset was pre-processed (augmented) by adding images that were distorted in different ways.
The MNIST dataset was famously published, but the augmented dataset was not. 
The DNN and CNN algorithms were implemented without relying on an open source library while \emph{initialization} of the experiment included the initialization of neural network weights was done  manually by hand as well more systematically for different parts. 
It is not clear whether the complete \emph{workflow} was automated or parts of it were done manually, as code is not shared.  
\emph{Ancillary software}, such as operating system, was not specified, but the \emph{hardware} was, as the experiment was executed on a Silicon Graphics Origin server with a 200 MHz F10000 processor.
Executing the training of the algorithms on the training data resulted in the two models $m_{DNN}$ $m_{CNN}$.

The \emph{outcome} is the classes [0-9] given to each image in the test set. 
It is not shared, but the \emph{analysis} is, which is the metric error rate (in \%) on the test set reported in a bar graph. 
The best DNN has an error rate of 2.95\% without training on distorted images and an error rate of 2.45\% when the distorted images are used while the best CNN (LeNet-5) has an error rate of 0.95\% that is reduced to 0.8\% when adding distortion. 
Non-neural network baselines were also reported, which includes SVM's among several others. 
The best baseline reported a result of 0.8\%.
The uncertainty is reported to be 0.1\% for all the error rates. 
However, it is not clear how the uncertainty is computed.
The alternative hypothesis is supported as the CNN is better than DNN taking the uncertainty into account.
However, the experiment cannot conclude what the state of the art is performance-wise, as the experiment has no clear winner given how close the error rate of the SVM and CNN are. 
Still, additional experiments show that the CNN runs faster and requires less memory, which are important properties when choosing algorithms. 
%\oeg{Should I integrate the six factors more explicitly in this example: Study design, algorithmic, implementation, observation, evaluation, documentation into this example.}




%A model comparison study is conducted where two machine learning models, $m_a$ and $m_b$, compete to identify which of them are better at performing a classification task. %$m_{DNN}$ $m_{CNN}$
%The hypothesis is that $m_a$ performs better than $m_b$ on the test dataset after being trained on the training dataset.
%10-fold cross validation is done to identify the best set of hyperparameters for each model.
%After identifying the best hyperparameters each of the models classify each image in the test set.
%Performance is measured using classification error.
%The experiment is run five times and the mean error and variance are reported.
%The strength of the evidence is measured through statistical hypothesis testing.
%The final results support the hypothesis in that $m_a$ performs significantly better than $m_b$.
%The conclusion from the original study was that it supports the hypothesis. 




%Things to discuss:
%- The task of the model comparison experiment => define properly in related to the definition
%- Data
%- ML methodology
% Engineering


% Stuff commented out: Draft ideas
%Machine learning methodology is developed around the notion that "an agent learns if it improves its performance after making observations about the world" \cite{russel_norvig_2020}. 
%In supervised learning, which is the most common form of machine learning algorithms, agents learn from input-output pairs and have to learn to map input to output, and its performance is measured using a performance metric such as error rate, that is the proportion of times where the agent fails to map the input to the output.



%artificial Intelligence, and machine learning by extension, is not only about studying the behavior of intelligent systems, but also to build them \cite{russel_norvig_2020}.


%While the performance of some systems are evaluated on their performance on real-world tasks, such as AlphaGo and Watson
%While some ML systems are built and evaluated 



